Cascades and Obstructions of Low Connectivity for Embedding Graphs into the Klein Bottle

The structure of graphs with a 2-vertex-cut that are critical with respect to the Euler genus is studied. A general theorem describing the building blocks is presented. These constituents, called hoppers and cascades, are classified for the case when Euler genus is small. As a consequence, the complete list of obstructions of connectivity 2 for embedding graphs into the Klein bottle is obtained.

==> amsdef.tex <==
%Amsdef LaTex template 

\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}


%---------------------------- repeated theorem -----------------------------
%http://tex.stackexchange.com/questions/422/how-do-i-repeat-a-theorem-number

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}

%----------------------------- problem-def -------------------------------
\newtheoremstyle{problem-def}%
{}%	Space above 
{}%	Space below 
{}%	Body font
{}%	Indent amount
{\sc}% Theorem head font 
{.}%	Punctuation after theorem head 
{.5em}%	Space after theorem head2 
{\thmnote{#3}}%	Theorem head spec (can be left empty, meaning normal)
\theoremstyle{problem-def}
\newtheorem*{problem-def}{Problem}
\theoremstyle{plain}


